Argument Linking: A Survey and Forecast

Semantic role labeling (SRL) -- identifying the semantic relationships between a predicate and other constituents in the same sentence -- is a well-studied task in natural language understanding (NLU). However, many of these relationships are evident only at the level of the document, as a role for a predicate in one sentence may often be filled by an argument in a different one. This more general task, known as implicit semantic role labeling or argument linking, has received increased attention in recent years, as researchers have recognized its centrality to information extraction and NLU. This paper surveys the literature on argument linking and identifies several notable shortcomings of existing approaches that indicate the paths along which future research effort could most profitably be spent.

==> sections/background/uds.tex <==
The Universal Decompositional Semantics (UDS) initiative provides a semantic layer on top of the Universal Dependencies (UD) dependency graphs for the English Web Treebank, and is broadly motivated by arguments from linguistic theory that word meanings are best understood \textit{decompositionally}---that is, as entities that may be factored into sets of simpler properties. The project augments the English Web Treebank with sentence-level semantic graphs, commonsense semantic annotations on those graphs, and a toolkit for working with both. Each of these components is presented in detail below.

\subsubsection{Sentence-level semantic graphs}
The nodes of the semantic graphs are predicates and arguments and the edges indicate which arguments belong to which predicates. These relations are extracted using PredPatt, a lightweight tool that relies on deterministic, unlexicalized rules to identify these relations directly from the UD dependency graphs. [DESCRIPTION OF HOW PREDPATT WORKS]

\subsubsection{Annotations}
Arguably the most valuable facet of UDS is its rich set of annotations. Collectively, these constitute the UDS1.0 dataset and cover a broad range of semantic properties, collected from native English speakers on Amazon Mechanical Turk through questions posed in plain language. The questions are organized into \textit{protocols}, each related to a distinct set of semantic phenomena, and do not require any linguistic expertise to answer. Figure FIGURE shows an example interface from the word sense protocol. Table TABLE shows a complete list of the protocols in UDS1.0, along with short descriptions of each.


\subsubsection{Toolkit}

The Decompositional Semantics 
